Challenges for dark matter direct search with SiPMs

Liquid xenon and liquid argon detectors are leading the direct dark matter search and are expected to be the candidate technology for the forthcoming generation of ultra-sensitive large-mass detectors. At present, the scintillation light detection in those experiments is based on ultra-pure low-noise photo-multipliers. To overcome the issues in terms of the extreme radio-purity, costs, and technological feasibility of the future dark matter experiments, the novel SiPM-based photo-detector modules look promising candidates, capable of replacing the present light detection technology. However, the intrinsic features of SiPMs may limit the present expectations. In particular, interfering phenomena, especially related to the optical correlated noise, can degrade the energy and pulse shape resolutions. As a consequence, the projected sensitivity of the future detectors has to be reconsidered accordingly.

==> pkgs.tex <==
\makeatletter
\@ifpackageloaded{natbib}{}{\usepackage{cite}}

\@ifpackageloaded{hyperref}{}{\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}}

\@ifundefined{oldSI}{%
\usepackage[separate-uncertainty,retain-explicit-plus,per-mode=symbol,product-units=power,range-units = single]{siunitx}
}{%
\usepackage[separate-uncertainty,retain-explicit-plus,per-mode=symbol,product-units=power,range-units = single]{siunitx}[=v2]
\newcommand\qty{\SI} %compatibility for arxiv
\newcommand\qtyproduct{\SI}
\newcommand\qtyrange{\SIrange}
}
\makeatother

\DeclareSIUnit\cps{cps}
\DeclareSIUnit\electron{\mbox{$e^-$}}
\DeclareSIUnit\eVee{\mbox{eV$_{ee}$}}
\DeclareSIUnit\eVnr{\mbox{eV$_{nr}$}}
\DeclareSIUnit\barg{barg}
\DeclareSIUnit\oV{OV}
\usepackage{lineno}
\usepackage{isotope}

\setlength{\marginparwidth}{2cm}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc} 
%\usepackage{appendix}
\usepackage{todonotes}
\usepackage{amssymb}
\usepackage{amsmath}
\usepackage{wasysym}
\usepackage{nicefrac}
\usepackage{tabularx}
\usepackage{listings}


%\usepackage{titlesec}
%\titlespacing{\subsection}{0pt}{1.2\baselineskip}{0.8\baselineskip}

%\usepackage{caption}
%\captionsetup[table]{position=bottom}

\DeclareMathSymbol{\mdot}{\mathord}{symbols}{"01}

\newcommand{\task}[1]{\todo[inline]{#1}}
\newcommand{\unsure}[1]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,inline]{#1}}
\newcommand{\change}[1]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,inline]{#1}}
\newcommand{\info}[1]{\todo[linecolor=OliveGreen,backgroundcolor=OliveGreen!25,bordercolor=OliveGreen,inline]{#1}}
\newcommand{\improvement}[1]{\todo[linecolor=Plum,backgroundcolor=Plum!25,bordercolor=Plum,inline]{#1}}

